Market Making with Decreasing Utility for Information

We study information elicitation in cost-function-based combinatorial prediction markets when the market maker's utility for information decreases over time. In the sudden revelation setting, it is known that some piece of information will be revealed to traders, and the market maker wishes to prevent guaranteed profits for trading on the sure information. In the gradual decrease setting, the market maker's utility for (partial) information decreases continuously over time. We design adaptive cost functions for both settings which: (1) preserve the information previously gathered in the market; (2) eliminate (or diminish) rewards to traders for the publicly revealed information; (3) leave the reward structure unaffected for other information; and (4) maintain the market maker's worst-case loss. Our constructions utilize mixed Bregman divergence, which matches our notion of utility for information.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\miro{This paper analyzed settings
when the schedule of the value of information
is known ahead of time. However, some of the ideas
in this paper might be applicable to adaptive
settings, e.g., those studied by \citet{B+12}
in the Bayesian setting. Here tho goal
is to detect ``high information''
periods based on the trading behavior.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "seq_mm"
%%% End:

